Your Semantic-Independent Watermark is Fragile: A Semantic Perturbation Attack against EaaS Watermark

Embedding-as-a-Service (EaaS) has emerged as a successful business pattern but faces significant challenges related to various forms of copyright infringement, particularly, the API misuse and model extraction attacks. Various studies have proposed backdoor-based watermarking schemes to protect the copyright of EaaS services. In this paper, we reveal that previous watermarking schemes possess semantic-independent characteristics and propose the Semantic Perturbation Attack (SPA). Our theoretical and experimental analysis demonstrate that this semantic-independent nature makes current watermarking schemes vulnerable to adaptive attacks that exploit semantic perturbations tests to bypass watermark verification. Extensive experimental results across multiple datasets demonstrate that the True Positive Rate (TPR) for identifying watermarked samples under SPA can reach up to more than 95\%, rendering watermarks ineffective while maintaining the high utility of embeddings. Furthermore, we discuss potential defense strategies to mitigate SPA. Our code is available at https://github.com/Zk4-ps/EaaS-Embedding-Watermark.

==> sections/acknowledgement.tex <==
% use section* for acknowledgment
\ifCLASSOPTIONcompsoc
  % The Computer Society usually uses the plural form
  \section*{Acknowledgments}
\else
  % regular IEEE prefers the singular form
  \section*{Acknowledgment}
\fi


We would like to appreciate all anonymous reviewers for their insightful feedback and constructive suggestions to improve this work. This work was supported by the Key Laboratory of Data and Intelligent System Security Ministry of Education, Nankai University, China. 




==> sections/useless.tex <==
\textbf{Finding 1: Differences in Similarity.} We begin by focusing on the dataset $D_c$ used by the attacker. Assuming the corresponding non-watermarked embedding set $E^{o}_c$ is accessible. The semantic differences within any two samples $\{(d_{c_i}, d_{c_j})|i, j \in |D_c|\}$ in $(D_c, E^{o}_c)$ lead to varying cosine similarities between their corresponding original embeddings $\{(e^{o}_{c_i}, e^{o}_{c_j})|i, j \in |E^{o}_c|\}$. The cosine Similarity distribution can be approximated as a normal distribution. Specifically, $D_c$ can be divided into $D^t_c$ and $D^{wt}_c$ based on whether they contain the triggers, following the mid-frequency tokens selection rules in EmbMarker and WARDEN. Thus, $(D_c, E^{o}_c)$ can be also divided into $(D^t_c, E^{t_{o}}_c)$ and $(D^{wt}_c, E^{wt_{o}}_c)$. Embedding pairs $(e^{t_{o}}_{c_i}, e^{t_{o}}_{c_j})$ and $(e^{wt_{o}}_{c_i}, e^{wt_{o}}_{c_j})$ are iteratively and randomly selected from the two sets, with their cosine similarities computed at each iteration. Then, we can obtain a cosine similarity distribution containing the ground truth, as shown in Figure \ref{fig_1:image1}. 



\begin{figure}[!t]
    \centering
    \subfloat[Original]{%
        \includegraphics[width=0.20\textwidth]{figures/ground_truth_cos.png}
        \label{fig_1:image1}
    }
    \hspace{0.03\textwidth}
    \subfloat[Actual]{%
        \includegraphics[width=0.20\textwidth]{figures/ground_truth_cos_wm.png}
        \label{fig_1:image2}
    }
    \caption{Cosine Similarity Distribution with Ground Truth}
\label{fig_1}
\end{figure}


Figure \ref{fig_1:image1} presents the statistical results of randomly sampling the two sets for $10^6$ iterations, revealing almost complete overlap in their distributions. However, when the watermark is injected in the embedding set $(D^t_c, E^{o}_c)$ as EmbMarker. We repeat the random sampling for another $10^6$ iterations to compute the cosine similarities. The resulting distribution, as shown in Figure \ref{fig_1:image2}, exhibits a notable shift. This shift arises because the watermark injection scheme involves a fixed linear transformation that is inherently unrelated to the text semantic, leading to a substantial divergence between the two distributions. Such substantial divergence can only be observed with the ground truth. From the perspective of the attacker, as defined in Section \ref{sec:method_threat_model}, the attacker is unaware of the triggers and can only randomly select embedding pairs $(e^{o}_{c_i}, e^{o}_{c_j})$ from the entire dataset $(D_c, E^{o}_c)$. In this scenario, the probability that $(e^{o}_{c_i}, e^{o}_{c_j})$ simultaneously contains the watermark is extremely low. So it is difficult for the attacker to detect the suspicious samples from the distribution, as illustrated in Figure \ref{fig_2}.

\begin{figure}[!t]
\centering
\includegraphics[width=2in]{figures/attacker_cos_wm.png}
\caption{Cosine Similarity Distribution without Ground Truth}
\label{fig_2}
\end{figure}






However, from the attacker's perspective, the attacker is unaware of the triggers. The probability of randomly selecting watermarked embedding pairs from $(D_c, E^{o}_c)$ is very low. Consequently, the attacker aims to enhance the shift to make it more apparent from their perspective. This distribution shift enables the identification of potentially suspicious samples in $D_c$ that may contain triggers. According to the threat model, the attacker can access the original EaaS service $S_v$, enabling them to construct text pairs that contain triggers. A straightforward construction method: using a sample $d_{c_i}$ from $D_c$ and any other piece of text as $perb$. The attacker can create the text pair $(d_{c_i}, d_{c_i} + perb)$. The notation `+' represents the concatenation of the two text segments. We define $d'_{c_i} = d_{c_i} + perb$ and $e'_{c_i} = e^{perb}_{c_i}$. For the text pair $(d_{c_i}, d_{c_i} + perb)$, the portion of the text $d_{c_i}$ is identical. Therefore, whether $d_{c_i}$ contains triggers will influence the cosine similarity of the corresponding embedding pair $(e_{c_i}, e'_{c_i})$. If $d_{c_i}$ contains triggers, the cosine similarity of $(e_{c_i}, e'_{c_i})$ is expected to fall within an abnormal distribution. We propose two perturbation benchmarks.







According to the threat model, the attacker cannot acquire any information about the triggers. Thus, the concatenated suffix may contain triggers, ultimately impacting the performance of the perturbation. This situation is unavoidable, as the attacker lacks access to the service provider's relevant knowledge. Therefore, regardless of the perturbation method used, we select $k$ samples as suffixes for perturbation. Mid-frequency tokens are typically selected as triggers to minimize the impact on downstream task performance in backdoor-based watermarking schemes. Among the $k$ samples, only a limited number may carry triggers. So we combine the results from the $k$ trials to serve as the final evaluation metrics. 

\textbf{AUROC value based on cosine similarity of $(e_{c_i}, e'_{c_i})$:} Cosine similarity is an intuitive metric. It measures the difference between two high-dimensional vectors by using the cosine of the angle between them in vector space. We use the average of the $k$ trials as one of the evaluation metrics.

\textbf{AUROC value based on the $L_2$ distance of $(e_{c_i}, e'_{c_i})$:} $L_2$ distance, i.e., Euclidean distance represents straight-line distance between two points in high-dimensional space. The vectors $(e_{c_i}, e'_{c_i})$ are normalized and can be considered as lying on the unit circle in a high-dimensional space. Thus, the $L_2$ distance is related to the cosine similarity. As the angle between the vectors $\uparrow$, the cosine similarity $\downarrow$, and the $L_2$ distance $\uparrow$. We use the average of the $k$ trials as one of the evaluation metrics.

\textbf{AUROC value based on the PCA score of $(e_{c_i}, e'_{c_i})$:} Regardless of the perturbation method, we perform $k$ perturbations to mitigate the potential impact of triggers in the suffix. As a result, we obtain $e_{c_i}$ and $k$ perturbed embeddings: $\{ e^{j}_{c_i} \mid j=1,2,3,\ldots,k \}$. For each $d_{c_i}$, we obtain an embedding set $e^{set}_{c_i}$ of size $k+1$. We apply PCA to each set $e^{set}_{c_i}$, which serves as a dimensionality reduction algorithm for preprocessing high-dimensional data. By treating the space corresponding to $e^{set}_{c_i}$ as high-dimensional, we reduce its dimensionality and obtain eigenvalue for each principal component. If $d_{c_i}$ contains triggers, the embeddings in $e^{set}_{c_i}$ should be more clustered in high-dimensional space. After PCA, the lower-dimensional representation should also exhibit greater clustering, with significantly smaller eigenvalues. Therefore, we use the sum of the eigenvalues as one of the evaluation metrics.






\begin{itemize}
    \item If AUROC = 1, the classifier is a perfect classifier, meaning that there exists at least one threshold for which the predictions are flawless. 

    \item If 0.5 $<$ AUROC $<$ 1, the classifier performs better than random guessing. 

    \item If AUROC = 0.5, the classifier performs equivalent to random guessing. 

    \item If AUROC $<$ 0.5, the classifier performs worse than random guessing. If predictions are reversed, the model may perform better than random guessing.
\end{itemize}





\textbf{Semantic Perturbation Performance.} The performance of perturbation is the key to the success of SPA. We use the AUROC as the primary metric to evaluate the performance, as detailed in Section \textcolor{red}{!!!!}. We present the results for three different perturbation approaches. Note that each approach involves $k$ iterations of perturbation, with $k=10$ chosen to balance experiment time and cost considerations. 





(1) \textbf{\textit{Heuristic Perturbation Schemes}:} For a target sample $d_{c_i}$, we randomly select $k$ samples from $D_c$ with labels opposite to that of $d_{c_i}$ to form the candidate suffix set. Since our study focuses on text classification tasks, the texts in $D_c$ are labeled accordingly. For example, in a sentiment classification task, different labels correspond to positive and negative sentiments. Thus, texts with opposite labels can semantically perturb $d_{c_i}$. Finally, we combine the results from the $k$ perturbations to derive the evaluation metric. The results are shown in Table \ref{table_4}. The MIND dataset can be clearly separated into two groups based on the presence or absence of triggers. The heuristic approach achieves satisfactory perturbation performance, with AUROC values generally close to 0.95. However, the performance on the AG News dataset is suboptimal, as the method fails to identify suspicious samples selection and deletion. When employing the multi-target watermarking schemes like WARDEN, the triggers are divided into different groups. The groups anchor distinct target vectors, with orthogonal constraints applied across targets. Consequently, the Cosine AUROC and $L_2$ AUROC in the heuristic approach are significantly affected, as the watermark information added by WARDEN is less prominent compared to EmbMarker. Nonetheless, the PCA-based metric shows only a slight decrease because PCA extracts the primary components in the high-dimensional vector space, minimizing the impact of redundant information. Interestingly, the PCA AUROC on the SST2 dataset even increases slightly using the WARDEN scheme. This may be attributed to the inherent distribution characteristics of the SST2 dataset. 



\renewcommand{\arraystretch}{1.5}

\begin{table*}[!t]
\caption{Heuristic Perturbation Schemes Performance}
\centering
\begin{tabular}{c|c c c c c}
\hline
\textbf{Metrics} & \textbf{Schemes} & \textbf{Enron} & \textbf{SST2}  & \textbf{MIND} & \textbf{AG News}  \\ \hline
\multirow{2}{*}{Cosine AUROC} & EmbMarker & $0.9484$ & $0.9667$ & $1.0$  & $0.8670$ \\ 

& WARDEN & $0.8851$ & $0.9284$ & $0.999995$  & $0.8136$ \\ \hline

\multirow{2}{*}{$L_2$ AUROC} & EmbMarker & $0.9478$ & $0.9660$ & $1.0$  & $0.8668$ \\ 

& WARDEN & $0.8851$ & $0.9284$ & $0.999995$  & $0.8136$ \\ \hline

\multirow{2}{*}{PCA AUROC} & EmbMarker & $0.9554$ & $0.9413$ & $1.0$ & $0.8687$  \\ 

& WARDEN & $0.9233$ & $0.9546$ & $1.0$  & $0.8613$ \\  \hline

\end{tabular}
\label{table_4}
\end{table*}







(2) \textbf{\textit{Standard Model Suffix Perturbation Guidance}:} Using a small model $\Theta_s$ to guide the perturbation for a LLM-based model. We search for the $top$-$k$ suffixes $perb$ that maximize the difference in similarity between $(d_{c_i}, d_{c_i} + perb)$ and the corresponding $(se_{c_i}, se'_{c_i})$. The results from the $k$ perturbations are then combined to form the final evaluation metric. Although this approach is precise, it is inefficient. Therefore, we choose the candidate pool for perturbations as $D_c$, searching within the set itself for the optimal suffixes. The selected suffixes largely align with the heuristic approach. The majority of them having labels different from that of $d{c_i}$, as shown in Table \ref{table_5}. Table \ref{table_6} presents the perturbation metrics obtained using suffix perturbation guidance, demonstrating a significant improvement in the quality of the suffixes. In the same $D_c$, the perturbation behavior guided by the small model for the LLM-based model proves to be much more effective than random perturbations.


\renewcommand{\arraystretch}{1.5}

\begin{table}[!t]
\caption{Different Label Percentage in Suffix}
\centering
\begin{tabular}{c|c c c c}
\hline
\textbf{Schemes} & \textbf{Enron} & \textbf{SST2}  & \textbf{MIND} & \textbf{AG News}  \\ \hline
EmbMarker(label) & percentage  &  &   &  \\ 

WARDEN(label) &  &  &   &  \\ \hline

\end{tabular}
\label{table_5}
\end{table}






\renewcommand{\arraystretch}{1.5}

\begin{table*}[!t]
\caption{Standard Model Suffix Perturbation Guidance Performance}
\centering
\begin{tabular}{c|c c c c c}
\hline
\textbf{Metrics} & \textbf{Schemes} & \textbf{Enron} & \textbf{SST2}  & \textbf{MIND} & \textbf{AG News}  \\ \hline
\multirow{2}{*}{Cosine AUROC} & EmbMarker & $0.9838$ & $0.9821$ &   &  \\ 

& WARDEN &  &  &   &  \\ \hline

\multirow{2}{*}{$L_2$ AUROC} & EmbMarker & $0.9837$ & $0.9818$ &   &  \\ 

& WARDEN &  &  &   &  \\ \hline

\multirow{2}{*}{PCA AUROC} & EmbMarker &  &  &  &   \\ 

& WARDEN &  &  &  &  \\  \hline

\end{tabular}
\label{table_6}
\end{table*}





\renewcommand{\arraystretch}{1.5}

\begin{table*}[!t]
\caption{Standard Model Suffix Search Guidance Performance \textcolor{red}{change a direction}}
\centering
\begin{tabular}{c|c c c c c}
\hline
\textbf{Metrics} & \textbf{Schemes} & \textbf{Enron} & \textbf{SST2}  & \textbf{MIND} & \textbf{AG News}  \\ \hline
\multirow{2}{*}{Cosine AUROC} & EmbMarker & $0.992$ &  &   &  \\ 

& WARDEN &  &  &   &  \\ \hline

\multirow{2}{*}{$L_2$ AUROC} & EmbMarker & $0.991$ &  &   &  \\ 

& WARDEN &  &  &   &  \\ \hline

\multirow{2}{*}{PCA AUROC} & EmbMarker & $0.996$ &  &  &   \\ 

& WARDEN &  &  &  &  \\  \hline

\end{tabular}
\label{table_7}
\end{table*}









The attacker aims to enhance the embeddings' changes to make them more apparent, enabling the identification of potentially suspicious samples in $D_c$. Consequently, the attacker aims to enhance the embeddings' changes to make them more apparent, enabling the identification of potentially suspicious samples in $D_c$ that may contain triggers. According to the threat model, the attacker can access the original EaaS service $S_v$ to construct text pairs that both contain triggers. A straightforward construction method: using a sample $d_{c_i}$ from $D_c$ and any other text as $perb$. The attacker can create the text pair $(d_{c_i}, d_{c_i} + perb)$. The notation `+' represents the concatenation of the two text segments. We define $d'_{c_i} = d_{c_i} + perb$ and $e'_{c_i} = e^{perb}_{c_i}$. For the text pair $(d_{c_i}, d_{c_i} + perb)$, the portion of the text $d_{c_i}$ is identical. Therefore, whether $d_{c_i}$ contains triggers will influence the cosine similarity of the corresponding embedding pair $(e_{c_i}, e'_{c_i})$. If $d_{c_i}$ contains triggers, the similarity of $(e_{c_i}, e'_{c_i})$ is expected to fall within an abnormal distribution. 



The above example demonstrates a simple $d'_{c_i}$ construction method. $perb$ is concatenated as a suffix to $d_{c_i}$. There are various perturbation techniques (e.g., suffix concatenation, prefix concatenation, and synonym replacement). However, in EaaS scenario, the attacker is constrained to only two perturbation methods, i.e., prefix and suffix concatenation. The attacker should not alter $d_{c_i}$ itself during perturbation, as they lack the knowledge of the watermarking algorithm used by the EaaS provider and the specific triggers. Any modification within $d_{c_i}$ (e.g., synonym replacement), may cause the triggers in $d_{c_i}$ to be ineffective. If the trigger is rendered invalid, $e'_{c_i}$ may exhibit deviations, leading to a failed perturbation. Therefore, only two positions are suitable for $d_{c_i}$: as prefix or suffix.



Unless specified, all perturbations in the following sections are concatenating a suffix.





Moreover, it is both reasonable and realistic for EaaS providers and attackers to have access to a general text corpus $ D_p $. It is essential for the design of watermarking and attack schemes. For instance, in EmbMarker\cite{peng2023you} and WARDEN\cite{shetty2024warden}, providers select mid-frequency tokens from $ D_p $ as triggers.




\renewcommand{\arraystretch}{1.5}

\begin{table}[!t]
\caption{Selection and Deletion Rate \textcolor{red}{including all two percentage, we can use the confusion matrix}}
\centering
\begin{tabular}{c|c c c c}
\hline
\textbf{Schemes} & \textbf{Enron Spam} & \textbf{SST2}  & \textbf{MIND} & \textbf{AG News}  \\ \hline
EmbMarker(PCA) & percentage  &  &   &  \\ 

WARDEN(PCA) &  &  &   &  \\ \hline

\end{tabular}
\label{table_8}
\end{table}





Large Language Models (LLMs) (e.g., GPT\cite{radford2018improving}, BERT\cite{devlin2018bert}, GLM\cite{du2022glm} and PaLM\cite{chowdhery2023palm}) have achieved remarkable proficiency, driving significant advancements in Natural Language Processing (NLP) and seeing widespread adoption across diverse industries.

A critical component underlying LLMs advancements is embedding, which plays a pivotal role in representing the characteristics of text within LLMs and enabling effective learning and task execution.


Embedding-as-a-Service (EaaS) has emerged as a transformative paradigm, extending the capabilities of LLMs beyond traditional language processing. 

In EaaS, embeddings serve as outputs that power downstream tasks such as search, classification, and recommendation. 
Embeddings not only play a crucial role within NLP models (e.g., transformers), but also act as essential building blocks in multi-modal architectures. Multi-modal models utilize embeddings to represent various modalities (text, image, audio, etc.), facilitating the integration and linkage of diverse data sources. Additionally, embeddings are vital for constructing external knowledge repositories, including retrieval-augmented generation (RAG) and vector databases, where they enable efficient storage and retrieval of content across different formats.


As embedding techniques continue to evolve, the development and research dedicated to improving the quality and efficiency of embedding models have intensified. Leading companies, including OpenAI, NVIDIA, Alibaba, Microsoft, Amazon, and Google, actively contribute to this field with advanced models (e.g., text-embedding-ada-002, NV-Embed-v2, gte-Qwen2-7B-instruct, e5-mistral-7b-instruct, Titan-text-embeddings-v2 and Gecko-1b-768). \textcolor{red}{(have no idea how to abbreviate).} Community-driven platforms like HuggingFace have also established specialized embedding model leaderboards, such as MTEB (Multilingual Text Embedding Benchmark), which covers multiple languages including English, Chinese, French, Polish, and Russian. These developments highlight the global interest and competition in embedding advancements.


However, while existing watermarking schemes offer some degree of protection for embedding models' intellectual property (IP), they have no consideration of the text semantic. This limitation makes them vulnerable to sophisticated attacks that exploit semantic variations to bypass watermark detection. We introduce a new attack, known as the Semantic Perturbation Attack (SPA), which can effectively evade watermark verification by making obvious semantic changes to the text. To address this vulnerability, we propose Semantic Aware Watermark (SAW) scheme, a robust defense mechanism designed to resist attacks including SPA by injecting the watermark that adapt to text semantic. Our approach not only enhance the copyright protection of EaaS services but also aligns with regulatory requirements, such as the Safe and Secure Innovation for Frontier Artificial Intelligence Act (California) and EU Artificial Intelligence Act, which advocates for watermarking to indicate AI-generated content. By incorporating watermarks that are resilient to semantic perturbations, SAW offering a comprehensive solution for protecting the copyright of generative AI companies, also enabling the ability to mark and verify AI-generated outputs.

This paper presents a detailed exploration of SPA and SAW, demonstrating how SPA utilized the limitations of existing schemes and how SAW enhances the copyright protection of text embedding EaaS services. Furthermore, we believe that our approach can be extended to other applications, such as vector databases, thereby providing a robust framework for IP protection across various embedding scenarios. Additionally, SAW is model-unaware and can be implemented as a plug-in extension module. Our main contributions are as follows:

\begin{itemize}
\item We propose SPA (Semantic Perturbation Attack), a novel attack that bypasses the current watermarking schemes for EaaS, and we conduct extensive experiments to evaluate its effectiveness.

\item We introduce SAW (Semantic Aware Watermark) to strengthen backdoor-based watermarking by incorporating text semantic features. Our research indicates that SAW not only demonstrates resilience against semantic perturbation attacks (SPA) but also achieves greater stealth compared to previous schemes across a range of datasets.
\end{itemize}





\begin{figure*}[!t]
\centering
\includegraphics[width=0.8\textwidth]{figures/overview.png}
\caption{General Overview of The Framework}
\label{fig:overview}
\end{figure*}









